Towards Testing Monotonicity of Distributions Over General Posets

In this work, we consider the sample complexity required for testing the monotonicity of distributions over partial orders. A distribution $p$ over a poset is monotone if, for any pair of domain elements $x$ and $y$ such that $x \preceq y$, $p(x) \leq p(y)$. To understand the sample complexity of this problem, we introduce a new property called bigness over a finite domain, where the distribution is $T$-big if the minimum probability for any domain element is at least $T$. We establish a lower bound of $\Omega(n/\log n)$ for testing bigness of distributions on domains of size $n$. We then build on these lower bounds to give $\Omega(n/\log{n})$ lower bounds for testing monotonicity over a matching poset of size $n$ and significantly improved lower bounds over the hypercube poset. We give sublinear sample complexity bounds for testing bigness and for testing monotonicity over the matching poset. We then give a number of tools for analyzing upper bounds on the sample complexity of the monotonicity testing problem.

==> old_stuf.tex <==
\section{Actual Technical Write-up aka Notes from 6/16/16}
(contains some repetition from above, for completeness)


\section{Fixing a Distribution on Bipartite Graphs}

Let $G=(S,T,E)$ where $E \subseteq S \times T$ be an unweighted bipartite graph directed from $S$ to $T$, and consider a probability distribution $p$ on this poset. We define the \emph{violation} graph $\tilde{G}$ of $G$ as $\tilde{G} = (S, T, S\times T)$, a complete weighted bipartite graph, where the weight $w:(S\times T)\rightarrow \mathbb{R}^+ \cup \{0\}$ is given by $w(u, v) \triangleq \max\{p(u)-p(v), 0\}$. Roughly speaking, $(u,v)$ represents the non-monotonicity amount that needs to be fixed by decreasing $p(u)$, increasing $p(v)$, or a combination of both.

Consider the following construction. Let $\mathcal{M}(\tilde{G})$ be a maximum weight matching (MWM) of $\tilde{G}$. Create a probability distribution $q$ as follows: initially set $q = p$, then for each edge $(u,v) \in \mathcal{M}(\tilde{G})$ such that $p(u)>p(v)$ (i.e., $w(u,v)>0$), swap the probabilities assigned to $u$ and $v$.

\begin{theorem}
Given a probability distribution $p$ on a bipartite poset $G$, construct a probability distribution $q$ as described above. Then $q$ is a monotone probability distribution over $G$. Moreover, if $p$ is $\epsilon$-close to monotone in the total variation distance, then $d_{TV}(p,q) \leq 2\epsilon$.
\end{theorem}
\begin{proof}
Clearly $q$ is a probability distribution. Our theorem then follows from Lemma \ref{lem:matchapprox} and Lemma \ref{lem:matchvalid} given below.
\end{proof}
\begin{lemma}\label{lem:matchapprox}
$d_{TV}(p,q) \leq 2\epsilon$.
\end{lemma}
\begin{proof}
Let $w(M) \triangleq \sum_{(u,v)\in M} w(u,v)$ denote total weight of a matching $M$. Let $p'$ be a monotone distribution such that $d_{TV}(p,p') \leq \epsilon$. Then for any $(u,v) \in \mathcal{M}(\tilde{G}), p'(u) \leq p'(v)$. So \[|p(u)-p'(u)| + |p(v)-p'(v)| \geq p(u)-p(v) = w(u,v).\] Thus, \[w(\mathcal{M}(\tilde{G})) = \sum_{(u,v)\in M_{\tilde{G}}} w(u,v) \leq \sum_{(u,v)\in M_{\tilde{G}}} (|p'(u)-p(u)| + |p'(v)-p(v)|) \leq d_{TV}(p,p') \leq \epsilon\]
Now consider the constructed distribution $q$. For each $(u,v)\in M_{\tilde{G}}$, \[|p(u)-q(u)|+|p(v)-q(v)| = 2(p(u)-p(v)) = 2w(u,v).\]
Thus, \[d_{TV}(p,q) = \sum_{(u,v)\in \mathcal{M}(\tilde{G})} (|p(u)-q(u)|+|p(v)-q(v)|) \leq 2\mathcal{M}(\tilde{G}) \leq 2\epsilon,\]
as desired.
\end{proof}

\begin{lemma}\label{lem:matchvalid}
The probability distribution $q$ is monotone.
\end{lemma}
\begin{proof}
For simplicity of analysis, let us first assume that $G$ is balanced; i.e., $|S| = |T|$. Assume as well that $\mathcal{M}(\tilde{G})$ is a perfect matching; otherwise, we may extend it by adding edges of weight $0$. We define the following linear programming relaxation for MWM, where $x(u,v)$ is the indicator variable denoting whether $(u,v)$ is in the matching, but has been relaxed to allow fractional values. Unconventionally, our first two constraints allow the total $x(u,v)$ at each vertex to be smaller than $1$. This LP will later give a more convenient dual to work with. Since every $w(u,v)$ is non-negative in our case, decreasing any $x(u,v)$ never decreases the objective value. That is, our LP conserves the optimal value of the combinatorial MWM.

\begin{figure}[h]
\begin{center}
\begin{boxedminipage}{0.75\textwidth}
\underline{Maximum Weight Matching} (Primal)
\vspace{-0.05in}
\begin{align*}
	\text{maximize}& & \displaystyle\sum_{(u,v)\in S\times T} w(u,v) \cdot x(u,v) \\
	\text{subject to}& & \displaystyle\sum_{u\in S} x(u,v) &\leq 1 && \forall v \in  T \\
	& & \displaystyle\sum_{v\in S} x(u,v) &\leq 1 && \forall u \in  S \\
	& & x(u,v) &\geq 0 && \forall (u,v) \in  S\times T
\end{align*}
\end{boxedminipage}
\end{center}
\vspace{-0.15in}
\caption{LP relaxation of the maximum weight matching problem.}
\label{fig:mwm-lp}
\end{figure}

Observe here that our LP is of the form $\max\{cx: x\in \mathcal{P}\}$ where $\mathcal{P} = \{x: Ax \leq b, x \geq 0\}$. Since $A$ is an incidence matrix of a bipartite graph, the polytope $\mathcal{P}$ is totally unimodular and, as this LP is clearly feasible, it has an integral optimal solution.\footnote{For more information on integral polyhedra, see e.g.~Chapter 5 of [KorteVygen].} Let $\hat{x}$ be the solution corresponding to the maximum weight matching $\mathcal{M}(\tilde{G})$, which must be optimal for this LP relaxation as well.

Next, consider the minimum weight vertex cover (MWVC) problem below, which is the dual of the MWM problem. The goal is to assign each vertex with a non-negative weight, so that for each edge $(u,v)$ the total values of the endpoints $y(u)+y(v) \geq w(u,v)$, while the total weight is minimized. Let $\hat{y}$ be an optimal solution to this LP.

\begin{figure}[h]
\begin{center}
\begin{boxedminipage}{0.75\textwidth}
\underline{Minimum Weight Vertex Cover} (Dual)
\vspace{-0.05in}
\begin{align*}
	\text{minimize}& & \displaystyle\sum_{u\in S} y(u) + \sum_{v\in T} y(v) \\
	\text{subject to}& & y(u) + y(v) &\geq w(u,v) && \forall (u,v)\in S\times T \\
	& & y(u) &\geq 0 && \forall u \in  S \\
	& & y(v) &\geq 0 && \forall v \in  T
\end{align*}
\end{boxedminipage}
\end{center}
\vspace{-0.15in}
\caption{LP relaxation of the minimum weight vertex cover problem.}
\label{fig:mwvc-lp}
\end{figure}

Next we show that $q(u) \leq q(v)$ for every $(u,v)$ of $G$. Firstly consider the case where $(u,v)$ is originally monotone with respect to $p$: $p(u) \leq p(v)$. Since we only swap edges that are non-monotone with respect to $p$, we have $q(u) \leq p(u)$ and $q(v) \leq p(v)$. Thus $q(u) \leq p(u) \leq p(v) \leq q(v)$; that is, $(u,v)$ is monotone with respect to $q$.

Now, recall the complementary slackness condition $(\hat{y}(u) + \hat{y}(v)-w(u,v))\cdot \hat{x}(u,v)=0$ as $\hat{x}, \hat{y}$ are optimal for their respective LPs. Since $\hat{x}(u,v) = 1$ for $(u,v) \in \mathcal{M}(\tilde{G})$, we have the tight condition $\hat{y}(u)+\hat{y}(v) = w(u,v)$. As $\hat{y}(u),\hat{y}(v) \geq 0$, we have that $\hat{y}(u), \hat{y}(v) \leq w(u,v)$. So,
\[
q(u)=p(v)=p(u)-w(u,v)\leq p(u)-\hat{y}(u) \textrm{ and } q(v)=p(u)=p(v)+w(u,v)\geq p(v)+\hat{y}.\]
These conditions apply to all $u\in S$ and $v\in T$ because all vertices are matched, by our assumption that $\hat{x}$ corresponds to a perfect matching.

Consider now any edge $(u,v) \in G$ (not necessarily in $\mathcal{M}(\tilde{G})$) that is not monotone with respect to $p$: $p(u)>p(v)$. From the analysis above we have
\begin{align*}
q(u) \leq p(u)-\hat{y}(u) \leq p(u)-(w(u,v)-\hat{y}(v)) = p(u)-(p(u)-p(v))+\hat{y}(v)=p(v)+\hat{y}(v)\leq q(v),
\end{align*}
so $q$ is monotone with respect to $G$, as desired.

Finally, via a reduction, we relax our initial assumption that $G$ is balanced. We construct an auxiliary graph $G'$ from $G$ by adding vertices to the part with smaller number of vertices until $G'$ becomes balanced. The distribution $p'$ is the same as $p$ for vertices of $G$. When $|S| < |T|$, assign $p'(u)=0$ for each added vertex $u$. When $|T| > |S|$, assign $p'(v)=1$ to each added vertex $v$. Note that $p'$ is not necessarily a probability distribution, but this does not affect our analysis above. We define the violation graph $\tilde{G'}$ of $G'$ accordingly.

Observe that every edge incident to any added vertex has weight $0$ by construction. So, the matching $\mathcal{M}(G)$ on $\tilde{G}$ may be extended to a matching $\mathcal{M}(\tilde{G'})$ on $\tilde{G'}$ of the same weight. We may then apply the argument above on the balanced bipartite graph $G'$ and MWM $\mathcal{M}(\tilde{G'})$, yielding distribution $q'$. All added edges are monotone with respected to $p'$, so $q'$ does not swap any added vertices; that is, it swaps exactly the same pair of vertices as $q$ does on $p$. As all edges of $G'$ becomes monotone with respect to $q'$, so do edges of $G$ with respect to $q$. Therefore, $q$ is a monotone distribution over $G$.
%\todo[inline, color=blue!60]{Anak's bookmark}
\end{proof}


























\section{Basic reduction from [VV]}

\todo[inline, color=green!40]{Write down definitions}

\begin{defn}
A probability distribution $p$ is called $T$-\emph{big} if all probabilities in the distribution are at least $T$.
\end{defn}

For example, the uniform distribution is $1/n$-big. No distribution is $k/n$ big for $k>1$. All distributions are $0$-big.

\begin{lemma}
There exists a pair of distributions $(p_1,p_2)$ that take $\Omega(n/\log n)$ to distinguish using fingerprints, such that
\begin{itemize}
\item $p_1$ is $T$-big (say threshold $T$, think of something like $1/(100n)$) and $p_2$ is $\epsilon$-far from being $T$-big.
\item The maximum probability of any element in either distributions is $O(\textrm{polylog}(n) / n)$ {\color{red} something like $(\log k) / k$ when $k = n / \log n$, so this is probably more like $(\log^2 n)/n$}
\end{itemize}
\end{lemma}

\todo[inline, color=green!40]{Write down explicitly where we got these facts from VV. Also, describe the relationship between testing support size and testing bigness.}

Theorem 1 from [VV] shows that ``for any positive constant $\phi < \frac{1}{4}$, there exists a pair of distributions $p^{F+}$ and $p^{F-}$ that are $O(\phi |\log \phi|)$-close in the relative earthmover distance, respectively, to the uniform distributions on $n$ and $\frac{n}{2}$ elements (where $n_\textrm{VV} = \frac{32}{\phi} k \log k$), but which are indistinguishable to $k = \frac{\phi}{32} \cdot \frac{n_\textrm{VV}}{\log n_\textrm{VV}}$-sample testers.'' Here the chosen parameters are chosen such that $k \log k = \Omega(n)$ and $\phi |\log \phi| = \epsilon$. In particular, $k = \frac{n_\textrm{VV}}{\log n_\textrm{VV}}$ and $\phi |\log \phi| = \epsilon$ works. {\color{red} $\phi |\log \phi|$ is increasing for $\phi \in (0, \frac{1}{4})$, so the bound is weaker when $\epsilon$ is smaller?}

By construction according to Definition 12, two zeroes of $M_{j, \phi}(x)$ are at $\frac{\phi}{j}$ and $\frac{2\phi}{j}$ where $\phi < \frac{1}{4}$; the remaining zeroes are within the range $[\frac{1}{j}, 4j]$ due to Fact 11(2). Substituting $j = \log k$, all roots $x_i$ are within the range $[\frac{\phi}{\log k}, 4\log k]$. The probability masses are placed at probabilities $\frac{x_i}{32k}$, so all probabilities in this construction are within the range $[\frac{\phi}{32 k \log k}, \frac{\log k}{8k}]$. Also, note that there are at most $j+2 = \log k + 2$ roots; this is also the number of distinct probabilities assigned to any element.

After the fattening process according to Definition 17, the probability masses at probabilities $\frac{1}{k}, \frac{2}{k}, \ldots, \frac{\log k}{k}$ are created/increased. The range of possible probabilities becomes $[\frac{\phi}{32 k \log k}, \frac{\log k}{k}]$. This also increases the number of distinct probabilities to $2 \log k + 2$.

\paragraph{Closeness to Bigness}

As $p^{F+}$ is $O(\phi |\log \phi|)$-close to the uniform distribution (in the relative earthmover distance, which is bounded by the total variation distance distance (claimed in Definition 4)\footnote{Consider the total variation distance for moving a unit probability mass in a histogram from probability $x$ to $y$; without loss of generality assume $x \leq y$. The support size shrinks from $\frac{1}{x}$ to $\frac{1}{y}$, so the original mass of weight $x \cdot \frac{1}{y}$ does not need to be moved. Thus the total variation distance is $1-\frac{x}{y} \leq \ln \frac{y}{x}$. Accounting for the case where $x > y$ we have the upper bound of $|\ln \frac{x}{y}|$, the relative earthmover distance.}) where each element is of probability $\frac{\phi}{32 k \log k}$, at most $O(\phi |\log \phi|) / \frac{\phi}{32 k \log k} = O(k \log k |\log \phi|)$ elements from the support may be removed, leaving a support of size $n = n_\textrm{VV} - O(k \log k |\log \phi|) = n_\textrm{VV} - O(\frac{\epsilon k \log k}{\phi}) = n_\textrm{VV}(1 - O(\epsilon))$ since $\phi |\log \phi| = \epsilon$. So under the domain of size $n$, $p^{F+}$ is $T = \frac{\phi}{32 k \log k} = \frac{1}{n_\textrm{VV}} = \frac{1-O(\epsilon)}{n}$-big.

Similarly, $p^{F-}$ originally has support size $\frac{n_\textrm{VV}}{2} = \frac{16 k \log k}{\phi}$ which is then increased by at most $O(k \log k |\log \phi|)$. The new support size is $\frac{n_\textrm{VV}}{2}(1 + O(\epsilon)) = \frac{n}{2}(1+O(\epsilon))$. In other words, if $p^{F+}$ and $p^{F-}$ share the same domain of size $n$, then $\frac{n}{2}(1+O(\epsilon))$ elements of $p^{F-}$ has probability 0, while the rest has probability at least $T$. Thus it is $\frac{n}{2}(1-O(\epsilon)) T = \frac{n(1-O(\epsilon))}{2}\cdot\frac{(1-O(\epsilon))}{n} = (\frac{1}{2}-O(\epsilon))$-far from $T$-bigness.

{\color{red} In particular, if $\epsilon$ is a sufficiently small constant, then $p^{F+}$ is $\frac{n}{100}$-big and $p^{F-}$ is $\epsilon$-far from being $\frac{n}{100}$-big. This is a little ``wasteful'' though.}

\paragraph{Sampling Complexity}

$k = \frac{\phi n_\textrm{VV}}{\log n_\textrm{VV}} = \frac{\phi n/(1-O(\epsilon))}{\log (n/(1-O(\epsilon)))} = \frac{(1+O(\epsilon))\phi n}{\log n - \log(1-O(\epsilon))}$ {\color{red} $\approx \frac{(1+O(\epsilon))\phi n}{\log n} = O(\frac{n}{\log n})$ for small constant $\epsilon$. Also, since $\phi |\log \phi|$ is increasing for $\phi \in (0, \frac{1}{4})$, the performance is better when $\epsilon$ is smaller?}

\paragraph{Maximum Probability}

As discussed above, the maximum possibility would be $\frac{\log k}{k} = \frac{\log (\phi n_\textrm{VV}) - \log (32 \log n_\textrm{VV})}{\phi n_\textrm{VV} / (32 \log n_\textrm{VV})} = O(\frac{\log \phi + \log^2 n_\textrm{VV}}{\phi n_\textrm{VV}})$ {\color{red} $\approx O(\frac{\log \phi + \log^2 n + \log^2 (1+O(\epsilon))}{(1+O(\epsilon)) \phi n}) = O(\frac{\log^2 n}{n})$ for small constant $\epsilon$.}

{\color{red}
\paragraph{Rounding Issues}

Here, we have been assuming that $p^{F+}$ and $p^{F-}$ corresponds to actual distributions, but in fact, the probability mass at some probability may not be a multiple of that probability. Say suppose we use rounding, then our analysis of the support size may be off by an additive error of $2 \log k + 2 \ll n$ if rounding affects the support size by an additive constant per "bar" of the histogram.
}

\begin{corollary}[follows directly from lemma]
Testing bigness requires $\Omega(n/\log n)$ samples.
\end{corollary}

\begin{corollary}[matching]
construct a matching: scaling factor $=1/(1+Tn)$, becomes $\epsilon' = \epsilon/(1+Tn)$-far from monotone
\end{corollary}

For the hypercube on $N$ vertices, we embed a matching of size $n = \Theta(N / \sqrt{\log N})$ into the hypercube. In order to preserve monotonicity, we set the probability of every element ``above'' the embedding in the hypercube to the maximum probability of any element we embed. Then, we rescale to make the probabilities sum to $1$. This gives the following lower bound.


\todo[inline, color=green!40]{Write down the construction and carefully prove it. Hopefully pin down the dependence on $\epsilon$. Substitute that to see actual dependence on $N$}

\begin{lemma}[hypercube]
can plug this construction into a Boolean hypercube; this becomes
\[\epsilon''=\frac{\epsilon}{(1+Tn) \cdot \textrm{The maximum probability of any element in either distributions} \cdot N}=\frac{\epsilon}{c' \sqrt{\log N}}\]
-far from monotone; lower bound is $\Omega(N/\log^{1.5} N)$ but this is with a nonconstant $\epsilon$ (as we have known) an assuming that the maximum probability is $O(1/n)$.
\end{lemma}

\begin{lemma} Let $p$ be a distribution over a matching of with $n = 2 {\log N - 1 \choose {\lfloor (\log N - 1)/2 \rfloor}}$ nodes such that the probability of each element is at monst $M$. If there exist an $\epsilon'$-test for monotonicity of distributions over hypercube with $N$ nodes, there exists an $\epsilon$-test for $p$.
\end{lemma}

\begin{proof}
To prove this lemma, we prove for a distribution $p$ over a matching, we can construct a distribution $p'$ over a hypercube such that the output of the $\epsilon'$-test for $p'$ be a valid output for an $\epsilon$-test for $p$. 


First, we  embed a matching with $n$ nodes into the hypercube. Thus, we need to find $n/2$ edges in hypercube which are mutually incomparable of each other. To do so, we pick all the nodes that among first $\log N - 1$ coordinates, there are exactly $\lfloor(\log N - 1)/2\rfloor$. Let $S$ denote the set of these points. There are exactly $n = 2 {\log N - 1 \choose {\lfloor (\log N - 1)/2 \rfloor}}$ nodes in the set $S$. It is not hard to see that each point in $S$ is comparable only with one other points which differs from it only in the last coordinate. Also, Each point is incomparable with the rest of the selected nodes, Since the number of ones in the first $\log N - 1$ coordinate is fixed. Thus, $S$ is the embeded matching into the hypercube.

Now, in order to construct the distribution $p'$ over the hypercube. We assign a weight to each node and then normalize the weight to sum up to one. For any node $x$ in $S$, let the weight of the $x$ be the $p(x)$. For any node $y$ that is comparable with any node in $S$, let its weight to be maximum probability in $p$ namely $M$. Finally, set the weight of rest of the nodes equal to zero. Now let $p'(x)$ be  $\mbox{weight}(x) / \sum_{y} \mbox{weight}(y)$. Based on definition it is clear that if $p$ is monotone then $p'$ is monotone. Also, if $p$ is $\epsilon$ far from being monotone, then $p'$ is at least $\epsilon' = \epsilon/ (M.N + 1)$ far from monotone. Thus, any $\epsilon'$-test for monotonicity of $p'$ is an $\epsilon$-test for monotonicity of the $p$.

\end{proof}


\iffalse
{\color{red} We're using a different $n$ here.}

\subsection{lower bound}

Say we embed a matching at $a := \frac{n}{2} \cdot b$ levels above the middle. Let $k = \frac{n}{2}+a$ be the level we embed the matching. While we aim at bounding ${n \choose k}$ against $\sum {n \choose j}$ for $j\in [k, n]$, we first consider only $j \in [k, k+a]$. Recall the ratio between consecutive terms of binomial coefficients in this range:
\[\frac{{n \choose j+1}}{{n \choose j}} = \frac{n-j}{j+1} \geq \frac{n-(k+a)}{(k+a)+1} = \frac{n-(\frac{n}{2}+nb)}{\frac{n}{2}+nb+1} \approx \frac{1-2b}{1+2b} \approx 1-4b\]
where inequality follows since the ratio is decreasing in $j$.
Then,
\[\sum_{j=k}^{k+a} {n \choose j} \geq {n \choose k} \sum_{i=0}^a  (1-4b)^i \approx {n \choose k} \frac{1-e^{-\Theta(n)}}{4b} \approx \frac{1}{4b} {n \choose k}.\]
Thus,
\[{n \choose k} \leq 4b \sum_{j=k}^{k+a} {n \choose j} \leq 4b \sum_{j=k}^{n} {n \choose k}.\]
%That is, the matching now constitutes a $\Theta(b)$-fraction of the non-zero weight of the hypercube, compared to the previous $1 / \sqrt{\log N}$ bound.

\subsection{upper bound}

Claim: can do $N^{1-c}$; do similar then upper bound the geometric series. Choose shifting amount: $\frac{n}{2} + c_1 n$. Pick $c_1$ really choose to $0$ so embedding size $N^{1-c_2}$ where $c_2 \rightarrow 0$ as $c_1 \rightarrow 0$.
\todo{prove}
\fi
\section{Constructing hard instances for bigness testing}

Construction: $x = y + V_L^{-1} V_R z$.

Claim: if probs $p_i = \alpha q_i$ then $V_R^t (V_L^{-1})t$ is diagonalizable. (proof: show full left eigenvectors exist, namely monomials) fact: left-right eigenvectors with different eivenvalues are orthogonal. So need to find eigenvectors orthogonal to those representing monomials $x^j$.

Pretty much known: we can match constant moments and $|y|$ is a multiple of $|z|$ (probably $k^k$).

Check valiant: use the same proof technique, derive that if I can match $k$ moments, then it takes $N^{1-1/k}$ samples to distinguish.

\subsubsection{One feasible solution ...}

\renewcommand{\vec}[1]{\mathbf{#1}}
\newcommand{\mat}[1]{\mathbf{#1}}

\begin{lemma}
Let $\mat{V_L}$ be the Vandermonde matrix whose rows are powers of $\vec{p} = \langle a+1, a+2, \ldots, a+k \rangle$ and let $\vec{w} = \langle 1, a, a^2, \ldots, a^{k-1}\rangle$. Then the vector $\hat{\vec{x}}$ where $\hat{x}_j = (-1)^{j+1} {k \choose j}$ for $j = 1, \ldots, k$ is the solution to the linear system $\mat{V_L}\hat{\vec{x}} = \vec{w}$.
\end{lemma}
\begin{proof}
We define polynomials $P_0(t) = (1-t)^k t^a$, and $P_{i}(t) = t\cdot\frac{d}{dt}P_{i-1}(t)$ for $i = 1, \ldots, k-1$. Via the binomial expansion, we have
\[P_0(t) = \sum_{j=0}^k {k \choose j} (-1)^{j} t^{a+j}.\]
By induction, we may verify that for $i=0, \ldots, k-1$,
\[P_i(t) = \sum_{j=0}^k (a+j)^i {k \choose j} (-1)^{j} t^{a+j}.\]
Observe that $1-t$ is a factor of $P_i(t)$ because $(1-t)^k$ is a factor of $P_0(t)$ and we apply the derivation $i < k$ times, so $P_i(t)=0$ when $t=1$. That is,
\[0 = P_i(1) = \sum_{j=0}^k (a+j)^i {k \choose j} (-1)^{j},\]
or equivalently,
\[\sum_{j=1}^k  (a+j)^i (-1)^{j+1} {k \choose j} = a^i.\]
That is, $\hat{x}_j = (-1)^{j+1} {k \choose j}$ satisfies every equation in the linear system.
\end{proof}

So, we can remove the negative terms of $\hat{\vec{x}}$ to $\vec{y}$ so that the vector representing the number of elements $\vec{x}, \vec{y}, \vec{z}$ are all non-negative and integral. Note that scaling so that the $L_1$-norm becomes $1$ can be done easily by dividing all probabilities by the first moment $\ell$: this scales down the $i$-th equation by a factor of $\ell^{-i}$, so the old solution will still satisfy this new system.

The above construction can be alternatively described as follows. We pick an integer $k > 1$ and a non-negative number $a$. Let $\ell$ be the normalization factor (to be specified). Then, the first $k$ moments (namely $0, \ldots, k-1$) of the following two distributions match. 
\begin{itemize}
\item Big distribution: for each odd $j$ in $0 \leq j \leq k$, there are $k \choose j$ elements of probability $(a+j)/\ell$;
\item Non-big distribution: for each even $j$ in $0 \leq j \leq k$, there are $k \choose j$ elements of probability $(a+j)/\ell$.
\end{itemize}
The normalization factor $\ell$ is the sum of the products ${k \choose j}(a+j)$ over either all odd $j$ or all even $j$:
\[\ell = \frac{1}{2}\left(\sum_{j=0}^k (a+j){k \choose j} \pm \sum_{j=0}^k (a+j){k \choose j} (-1)^{j}\right) = \frac{1}{2} \cdot \frac{d}{dt} \left((1+t)^k t^a\pm (1-t)^k t^a\right)\Bigr|_{t=1}=(k+2a)2^{k-2}.\]
Each of the distributions has a domain of size $n = 2^{k-1}$. All probabilities are $\Theta(1/n)$ (with an exception of probability $0$ when choosing $a=0$, for the one element corresponding to $j=0$ in the non-big distribution). Setting the threshold at $(a+1)/\ell$, the non-big distribution is $\epsilon = (1/\ell)$-far from $\frac{a+1}{\ell}$-bigness. The maximum probability of any element is $(a+k)/\ell$, so for the big distribution, the ratio between the maximum and minimum probabilities is at most $\frac{a+k}{a+1}$. When $a$ is large, this ratio decreases, but so does $\epsilon$.

\section{Old Sections that were removed/replaced}

\subsection{Lower Bound on Bigness Testing and on Monotonicity Testing on Matchings}

{\color{cyan}
Talk about the distribution constructed in WY: write all necessary parameters we'll need.
Show the construction to get Theorem 1: be sure to list all the issues we need to deal with, including showing big / far-from-big with desired parameters, and properly use the moments matching theorem.

}

{\color{red} Important paragraph, please read:}

Note that all we're doing in this subsection is going back through the proof of an existing lower bound in the literature and explaining that the proof still goes through unchanged if we want a lower bound on bigness instead of support size. IE., it's not just the techniques that aren't new: not even the proof itself is new.

\begin{defn}
A probability distribution $p$ is called $T$-\emph{big} if all probabilities in the distribution are at least $T$. The quantity $T$ is referred to as the \textit{bigness threshold}.
\end{defn}

This section is devoted to proving the following Theorem.

\begin{theorem}%\label{thm:bigness-lb}
For for some $T \in \Theta(1/n)$ and every $k \in \mathbb{N}$, there exists a pair $(C,S)$ of distributions of distributions on $[n]$ satisfying the following properties.
\begin{itemize}
\item $C$ always outputs $T$-big distributions.
\item $S$ outputs distributions that are $\epsilon$-far from $T$-big with probability 0.99, for some constant $\epsilon > 0$.
\item The ratio between the maximum probability over all possible distributions that may be output by either $C$ or $S$ over $T$ is $O(k^2)$.
\item The number of independent samples required to distinguish, with success probability $2/3$, a distribution chosen at random from either $C$ or $S$ is $\Omega(n^{1-\frac{1}{k+1}}/\log n)$.
\end{itemize}
In particular, if we make $k$ a sufficiently large constant, then the ratio of the max probability to the threshold is constant (and depends on $k$) and the exponent on $n$ in the lowerbound can be made arbitrarily close to $1$. For example, if we set $k=100$, we get $\epsilon=0.0001$ and a lower bound of $\Omega(n^{0.99})$.

Similarly, if we set $k=\log n$, the ratio of the max probability to the threshold is $O(\log^2 n)$ and we get a lower bound of $\Omega(n / \log n)$.
\end{theorem}

This lower bound is proven by constructing a pair of pseudo-distributions with matching fingerprint expectations. A pseudo-distribution is like a true probability distribution, except that elements are allowed to appear a fractional number of times:

\begin{defn}
A \textit{pseudo-distribution of size $n$} is a a pair of vectors $(a,p)$ each in $\mathbb{R}^n_{\geq 0}$ that satisfy $\sum_i a_i p_i = 1$ and $\sum a_i = n$.
\end{defn}

Intuitively, if we pair up the $i$th entries in the vectors $a$ and $p$, the pair $(a_i, p_i)$ means that there are $a_i$ elements each with probability $p_i$. If the $a_i$'s are all integral, then the pseudo-distribution is a true distribution. The notion of ``bigness'' can also be extended to pseudo-distributions since bigness only depends on what the probabilities are.

\begin{defn}
The \textit{$m$-sample $j$th fingerprint expectation} of a psuedo-distribution $p$ is defined as $\sum_i a_i \cdot \frac{(m p_i)^j e^{-m p_i}}{j!}$. We refer to $p$ as the \textit{probability vector} and $a$ as the \textit{frequency vector}.
\end{defn}

If the pseudo-distribution is also a true distribution, then its $m$-sample $j$th fingerprint expectation matches the standard definition; ie., the expected number of elements that are sampled $j$ times when we take $m$ samples.

Constructing pseudo-distributions with matching fingerprint expectations allows one to prove lower bounds on distribution testing/learning problems.

\textbf{TODO track down exact references or prove it explicitly}
\begin{theorem}[Implicit (maybe even explicit (?)) in DK and possibly WY]\label{thm:lb}
Suppose that there exists a pair of pseudo-distributions $(C_{\text{pseudo}}, S_{\text{pseudo}})$ each with (not necessarily the same) size $\Omega(n)$.\footnote{Without loss of generality, their sizes } Also suppose that the first $k$ $m$-sample fingerpint expectations are the same. Consider the pair of distributions of true distributions $(C,S)$ on $n$ elements defined as follows. A distribution output by $C$ ($S$) is generated as follows. Let $C_{\text{pseudo}}=(a,p)$ ($S_{\text{pseudo}}=(a,p)$). Independently assign each of the $n$ elements a probability, where the odds of assigning an element probability $p_i$ are proportional to $a_i$. Then, rescale the probabilities so that they sum to $1$.

Given $\Omega(\min(m,n^{1-\frac{1}{k+1}} / \log n))$ samples, no algorithm can tell whether the samples were drawn drawn from a distribution generated from $C$ or from $S$ with constant probability better $50\%$. {\color{red} $51\%$?}
\end{theorem}

% can we get away with matching slightly less than log n moments? (seems plausible)
% test monotonicity of levels, then use O(n/log n) matching pair learning inspired by that valiant paper
% 

By this theorem, we immediately get \autoref{thm:bigness-lb} provided we prove the following Lemma.\footnote{Note that the distributions of distributions $(C,S)$ described in \autoref{thm:lb} are not necessarily big or far from big with the same bigness threshold as that of the pseudo distributions $(C_{\text{pseudo}}, S_{\text{pseudo}})$. This is because we scale the probabilities to make them sum to $1$ when generating $C$ and $S$, which may cause the probabilities to be slightly smaller or larger than they were originally.

We can think of the scaling process as procedding in two steps: first, we scale the probabilities by the ratio of the size of the pseudo-distribution over the number of elements in the true distribution we are generating. This causes the expected sum of the probabilities in the true distribution to be $1$. Then, we scale 

However, the Chernoff bound implies that with probability $99\%$, we only have to scale (multiply or divide) them by a constant factor of at most $(1+\delta)$ for some $\delta \geq 0$. Furthermore, by making the domain size of the generated true distributions a sufficiently large constant factor larger than the size of the pseudo-distributions, we can make $\delta$ an arbitrarily small constant. So, we define $(C',S')$ to be the distributions of distributions conditioned on the event that we don't have to scale the probabilities by a factor larger than $(1+\delta)$---where $\delta$ is sufficiently small. No algorithm can distinguish samples drawn from them with constant probability better than $51\%$. Moreover, if we decrease the bigness threshold by a sufficiently small constant factor, $C'$ will always output big distributions and $S'$ will always output $\Omega(\epsilon)$-far from big distributions.
{\color{red} Just checking: no probabilities get scaled so max prob doesn't change, right? Only weights are scaled?}
}

\begin{lemma}[VV]
For every $m,k,n \in \mathbb{N}$, there exists a pair of pseudo-distributions on $n$ elements such that the first $k$ $m$-sample fingerpint expectations match and where one is $\Theta(1/n)$-big and the other is $\Omega(1/k^2)$-far from being $\Theta(1/n)$-big. Furthermore, the ratio between the maximum probability that can be output and the bigness threshold is $O(k^2)$.
\end{lemma}

This is proven in VV, so we are done.

\subsection{More failed stuff}

Consider the construction from Appendix F of [WY support]. Let $\lambda > 2$ be a real number and $k$ be a positive integer. There exists a pair of random variables $U, U'$ satisfying the following properties.
\begin{itemize}
\item $U, U' \in \{0\} \cup [2, \lambda]$
\item $E[U] = E[U'] = 1$
\item $E[U^i] = E[U'^i]$ for $i = 1, \ldots, k$
\item $P[U>0] - P[U'>0] = \frac{1-2\lambda^{-1}}{2}\left(\frac{\sqrt{\lambda}-\sqrt{2}}{\sqrt{\lambda}+\sqrt{2}}\right)^k$
\end{itemize}

First, we set $\lambda = c_1 k^2$ where $c_1$ is some absolute constant, so that $P[U>0] - P[U'>0] \geq d$ for some constant $d$. Next, define two random variables $V$ and $V'$ where $V$ is $U$ restricted to its nonzero domain elements and $V'$ is obtained by taking $U'$, subtracting $\Pr[U=0]$ from its probability of outputting $0$, and renormalizing to make it a probability distribution again. More specifically, let $z = P[U=0]$. Set $P[V = u] = \frac{P[U=u]}{1-z}$ for $u > 0$ (and $P[V = 0] = 0$, implying $V \in [2, \lambda]$), and $P[V'=u'] = \frac{P[U=u']}{1-z}$ for $u>0$ and $P[V'=0] = P[U'=0] - z$ .  Observe that $E[V^i] = E[V'^i]$ for $i = 1, \ldots, k$ as the probabilities of $V=0$ and $V'=0$ does not affect their moments, and other probabilities are scaled up by $\frac{1}{1-z}$, yielding $E[V^i]=E[U^i]/(1-z)^i$ and $E[V'^i]=E[U'^i]/(1-z)^i$, respectively. %Note that since $d \leq 1-z \leq 1$ and $d = \Omega(1)$, we have $1-z = \Theta(1)$.

Create two random vectors $P = \frac{1}{n} \langle V_1, \ldots, V_n\rangle$ and $P' = \frac{1}{n} \langle V'_1, \ldots, V'_n\rangle$, where $V_i$ and $V'_i$ are drawn independently from $V$ and $V'$, respectively. Observe that by the process above, $P[V>0]-P[V'>0] = P[V>0] = \frac{d}{1-z} \geq d$. Since $Var[V], Var[V'] \leq \frac{1}{4(1-z)^2}$, we apply Chebyshev's inequality (slightly adjusting the proof of Lemma 2 from [WY support]), yielding that for $\epsilon = \frac{4\lambda}{(1-z)\sqrt{n}}$, we have that $|\sum_{i=1}^{n} U_i -1|> \epsilon n$  with probabilty at most $\frac{1}{16}$, and $S(P) - E[S(P)] > \frac{nd}{4}$ with probability at most $\frac{16}{nd^2}$. The same two conditions apply for $P'$. We assume $\epsilon = O(1)$ as $n$ can be arbitrary large.

Now, we use the random vectors $P$ and $P'$ to generate Poissonized samples for our distributions $C$ and $S$; namely, $Poi(mU_i/n)$ samples are returned for $C$, and $Poi(mU'_i/n)$ samples are returned for $S$. While $P$ and $P'$ may not have unit $\ell_1$ norm, the first condition indicates that their norms are off by $\pm \epsilon$, which changes the total number of samples from $Poi(m)$ to $Poi(m')$ where $(1-\epsilon)m \leq m' \leq (1+\epsilon)m$. For $\epsilon = O(1)$, the algorithm still receives $\Theta(m)$ samples with high probability {\color{red} but it knows something about the scaling?}. The second condition implies that if we normailze $P$ and $P'$ to probability vectors, the minimum non-zero probability from these distributions are still at least $\frac{2}{1+\epsilon} \cdot \frac{1}{n} \geq \frac{1}{n}$ as $V, V' \in \{0\} \cup [2,\lambda]$. Lastly, we apply Lemma 3 of [WY new entropy] and obtain that for $k > 2e\lambda$, $TV(E[Poi(P)],E[Poi(P')]) \leq \left(\frac{2e\lambda}{k}\right)^k$. Choose ...

==> pream.tex <==
\makeatother\def\ni{\noindent}
% \newcommand{\secref}[1]{Section~\ref{#1}}
% \renewcommand{\cite}[1]{[{\tt{#1}}]}
\newcommand{\appref}[1]{Appendix~\ref{#1}}
%\newcommand{\mnote}[1]{ \marginpar{\tiny\bf
%            \begin{minipage}[t]{0.5in}
%              \raggedright #1
%          \end{minipage}}}
\newcommand{\mnote}[1]{}

%all kinds of tricks
\newcommand{\newparagraph}[1]{\noindent{\sf{#1}}}
\renewcommand{\paragraph}[1]{{\protect\vspace{8pt}\noindent\sc{#1}}}

%from BGS
\newlength{\saveparindent}
\setlength{\saveparindent}{\parindent}
\newlength{\saveparskip}
\setlength{\saveparskip}{\parskip}
\newenvironment{newitemize}{%
\begin{list}{$\bullet$}{\labelwidth=19pt%
\labelsep=7pt \leftmargin=12pt \topsep=3pt%
\setlength{\listparindent}{\saveparindent}%
\setlength{\parsep}{\saveparskip}%
% \setlength{\parsep}{1ex}
\setlength{\itemsep}{3pt} }}{\end{list}}

% \addtolength{\parskip}{0.5ex}              %separation between paragraphs


%shorthands for standard list-environments
\newcommand{\BE}{\begin{enumerate}} \newcommand{\EE}{\end{enumerate}}
\newcommand{\BI}{\begin{itemize}} \newcommand{\EI}{\end{itemize}}
\newcommand{\BDes}{\begin{description}}\newcommand{\EDes}{\end{description}}
% Theorem-like environments
\newtheorem{alg}{Algorithm}
\newcommand{\BA}{\begin{alg}} \newcommand{\EA}{\end{alg}}
%-----------------------------------------------------------------
\newtheorem{thm}{Theorem}[section]            % A counter for Theorems
% \newtheorem{thm}{Theorem}
\newcommand{\BT}{\begin{thm}} \newcommand{\ET}{\end{thm}}

% \newtheorem{lem}{Lemma}      % A counter for Lemmas
\newtheorem{lem}[thm]{Lemma} % Changed counter to be as for Theorems
\newcommand{\BL}{\begin{lem}} \newcommand{\EL}{\end{lem}}

\newtheorem{fact}{Fact}      % A counter for Lemmas
\newcommand{\BF}{\begin{fact}} \newcommand{\EF}{\end{fact}}
\newtheorem{clm}[thm]{Claim}
\newcommand{\BCM}{\begin{clm}} \newcommand{\ECM}{\end{clm}}

\newtheorem{techcor}[thm]{Corollary}
\newcommand{\BCo}{\begin{techcor}} \newcommand{\ECo}{\end{techcor}}

\newtheorem{cor}[thm]{Corollary}      % counter AS FOR Theorems
\newcommand{\BC}{\begin{cor}} \newcommand{\EC}{\end{cor}}
%%% CHANGE COUNTER so that PROPs go as THMs
\newtheorem{prop}[thm]{Proposition}     % A counter AS FOR Thms
% \newtheorem{prop}{Proposition}     % A counter AS FOR Thms
\newcommand{\BP}{\begin{prop}} \newcommand {\EP}{\end{prop}}
\newtheorem{conj} {Conjecture}      % counter AS FOR Theorems
\newcommand{\BCJ}{\begin{conj}} \newcommand{\ECJ}{\end{conj}}
%-----------------------------------------

\newtheorem{defn}{Definition}         % A counter for Definition
\newcommand{\BD}{\begin{defn}} \newcommand{\ED}{\end{defn}}
% \newtheorem{techdef}[lem]{Definition}
% \newcommand{\BDe}{\begin{techdef}}\newcommand{\EDe}{\end{techdef}}

% \newtheorem{definition}{Definition}
% \newtheorem{lemma}{Lemma}
% \newtheorem{theorem}{Theorem}

%referring to Theorems, etc.
%\newcommand{\eqref}[1]{Eq.~(\ref{#1})}
%\newcommand{\thmref}[1]{Theorem~\ref{#1}}
%\newcommand{\lemref}[1]{Lemma~\ref{#1}}
%\newcommand{\propref}[1]{Proposition~\ref{#1}}
\newcommand{\clmref}[1]{Claim~\ref{#1}}
%\newcommand{\corref}[1]{Corollary~\ref{#1}}

%%%%%%% Proof Environments
\def\FullBox{\hbox{\vrule width 8pt height 8pt depth 0pt}}
\newcommand{\qed}{\;\;\;\FullBox}
\newcommand{\ourqed}{\;\;\;\FullBox}
\newenvironment{ourproof}{\noindent{\bf Proof:~~}}{\(\ourqed\)}
\newcommand{\BPF}{\begin{ourproof}} \newcommand {\EPF}{\end{ourproof}}
\newenvironment{proofof}[1]{\noindent{\bf Proof of {#1}:~~}}{\(\qed\)}
\newcommand{\BPFOF}{\smallskip \begin{proofof}} \newcommand {\EPFOF}{\end{proofof}}
\newcommand{\qedsketch}{\;\;\;\Box}
\def\blackslug
{\hbox{\hskip 1pt\vrule width 8pt height 8pt depth 1.5pt\hskip 1pt}}
%\def\qed{\quad\blackslug\lower 8.5pt\null\par}
\def\qqed{$\Box$}

\newenvironment{smallproof}{\noindent{\bf Proof:~~}}{\(\qedsketch\)}
\newcommand{\bpf}{\begin{smallproof}} \newcommand{\epf}{\end{smallproof}}
%------------------------------------------------------------------------


%More Environments
\newcommand{\BEQ}{\begin{equation}} \newcommand{\EEQ}{\end{equation}}
\newcommand{\BEQN}{\begin{eqnarray}}\newcommand{\EEQN}{\end{eqnarray}}
% \newcommand{\BEQst}{\begin{equation*}} \newcommand{\EEQst}{\end{equation*}}
% \newcommand{\BEQNst}{\begin{eqnarray*}}\newcommand{\EEQNst}{\end{eqnarray*}}


%math macros
\newcommand{\eqdef}{\stackrel{\rm def}{=}}
\newcommand{\bitset}{\{0,1\}}
\newcommand{\bitsetn}{\{0,1\}^n}
\newcommand{\rnd}{\in_R}
% \newcommand{\th}{{\rm th}}
\newcommand{\st}{{\rm st}}
\renewcommand{\Pr}{{\rm Pr}}
\newcommand{\prob}{{\rm Prob}}
\newcommand{\Prob}{{\rm Prob}}
\newcommand{\exxp}{{\mbox{\bf\rm Exp}}}
\newcommand{\Exp}{{\mbox{\bf\rm Exp}}}
\newcommand{\var}{{\mbox{\bf\rm Var}}}
\newcommand{\Var}{{\mbox{\bf\rm Var}}}
\newcommand{\pr}{{\mbox{\bf\rm Pr}}}
\newcommand{\poly}{{\rm poly}}
\newcommand{\ov}{\overline}
\newcommand{\e}{\epsilon}
\newcommand{\eps}{\epsilon}
\newcommand{\da}{\delta}
\newcommand{\tildeO}{{\tilde{O}}}
\newcommand{\poi}{{\rm poi}}

%complexity classes
\newcommand{\NP}{{\cal NP}}
\newcommand{\BPP}{{\cal BPP}}
\newcommand{\RP}{{\cal RP}}
\newcommand{\coRP}{{\rm co}{\cal RP}}

\newcommand{\calO}{{\cal O}}
\newcommand{\calA}{{\cal A}}
\newcommand{\calC}{{\cal C}}
\newcommand{\calD}{{\cal D}}
\newcommand{\calF}{{\cal F}}
\newcommand{\calG}{{\cal G}}
\newcommand{\calH}{{\cal H}}
\newcommand{\calM}{{\cal M}}
\newcommand{\calP}{{\cal P}}
\newcommand{\calU}{{\cal U}}
\newcommand{\calPid}{{\cal P}^{\rm eq}}
\newcommand{\calPidmn}{{\cal P}^{\rm eq}_{m,n}}

\newcommand{\A}{{\rm A}}
\newcommand{\B}{{\rm B}}
\newcommand{\C}{{\rm C}}
\newcommand{\D}{{\rm D}}
\newcommand{\E}{{\rm E}}
\newcommand{\G}{{\rm G}}
\renewcommand{\H}{{\rm H}}
\newcommand{\I}{{\rm I}}
\newcommand{\K}{{\rm K}}
\renewcommand{\L}{{\rm L}}
\newcommand{\M}{{\rm M}}
\renewcommand{\O}{{\rm O}}
\newcommand{\Q}{{\rm Q}}
\renewcommand{\P}{{\rm P}}
\newcommand{\R}{{\rm R}}
\renewcommand{\S}{{\rm S}}
\newcommand{\T}{{\rm T}}
\newcommand{\W}{{\rm W}}
\newcommand{\U}{{\rm U}}
\newcommand{\V}{{\rm V}}
\newcommand{\X}{{\rm X}}
\newcommand{\Y}{{\rm Y}}

%%%%% ADDITIONAL LATEX MACROS
\newcommand{\sigmaone}{{\sigma_1}}
\newcommand{\dist}{{\rm dist}}
\newcommand{\dev}{{\rm dev}}
\newcommand{\argmax}{{\rm argmax}}
\def\xor{\oplus}
\newcommand{\newitem}{\vspace{-1ex}\item }
\newcommand{\emo}{\e_{\M}}
\newcommand{\dmo}{\da_{\M}}
\newcommand{\elin}{\e_{\sc lin}}
\newcommand{\dlin}{\da_{\sc lin}}
\newcommand{\floor}[1]{{\lfloor{#1}\rfloor}}
%
% \newcommand{\todo}[1]{\begin{quote}{\bf Note:} {\sc{#1}}\end{quote}}
% \newcommand{\todo}[1]{\iffalse {#1} \fi }

\newcommand{\po}{\prec}
\newcommand{\so}{\succ}

%\newcommand{\and}{\wedge}

\newcommand{\err}{{\rm err}}

\newcommand{\occ}{{\rm occ}}
\newcommand{\coll}{{\rm coll}}
\newcommand{\p}{{\mathbf p}}
\newcommand{\q}{{\mathbf q}}
\newcommand{\w}{\kappa}
\newcommand{\vbf}{{\mathbf v}}
\newcommand{\wbf}{{\mathbf w}}


\renewcommand{\And}{{\sc and}}
\newcommand{\Or}{{\sc or}}
\newcommand{\Xor}{{\sc xor}}

\newcommand{\infTest}{{\bf Bounded-$\ell_{\infty}$-Closeness-Test }}
\newcommand{\ltwoTest}{{\bf $\ell_2$-Distance-Test }}
\newcommand{\idtolTest}{{\bf Test-Tolerant-Identity }}
\newcommand{\loneTest}{{\bf $\ell_1$-Distance-Test }}
\newcommand{\lightTest}{{\bf TestLightIndependence }}
